Sampled-Data Online Feedback Equilibrium Seeking: Stability and Tracking

This paper proposes a general framework for constructing feedback controllers that drive complex dynamical systems to "efficient" steady-state (or slowly varying) operating points. Efficiency is encoded using generalized equations which can model a broad spectrum of useful objectives, such as optimality or equilibria (e.g. Nash, Wardrop, etc.) in noncooperative games. The core idea of the proposed approach is to directly implement iterative solution (or equilibrium seeking) algorithms in closed loop with physical systems. Sufficient conditions for closed-loop stability and robustness are derived; these also serve as the first closed-loop stability results for sampled-data feedback-based optimization. Numerical simulations of smart building automation and game-theoretic robotic swarm coordination support the theoretical results.

==> buildings.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{./figures/building.png}
  \caption{Example building generated via the BRCM toolbox~\protect\cite{sturzenegger2014brcm}.}
  \label{fig:building}
\end{figure}
% \begin{figure}
%   \centering
%   \begin{subfigure}[b]{\columnwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{./figures/rms.eps}
%     \caption{Temperature profile of the 5 rooms depicted in Figure~\protect\ref{fig:building}. Dashed lines indicate temperature bounds. \dlm{For space can we remove these captions? they're redundant with the axis labels, the part about the constraint bounds can go in the legend!}}
%     \label{fig:fb_opt_rooms}
%   \end{subfigure}\\
%   \begin{subfigure}[b]{\columnwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{./figures/rad.eps}
%     \caption{Power output of the radiators computed by feedback optimization. Dashed line indicates the hard input constraint.}
%     \label{fig:fb_opt_radiators}
%   \end{subfigure}\\
%   \begin{subfigure}[b]{\columnwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{./figures/ahu_af.eps}
%     \caption{AHU air flow computed by feedback optimization.}
%     \label{fig:fb_opt_ahu_flow}
%   \end{subfigure}
%   \vspace{0.25cm}
%   \caption{Simulation of the feedback optimization algorithm \protect\eqref{eq:PGM} on the building dynamics~\eqref{eq:1}.}
%   \label{fig:feedback_opt_results}
% \end{figure}
\begin{figure}[t]
  \centering
    \includegraphics[width=\columnwidth]{./figures/rms.eps}
    \includegraphics[width=\columnwidth]{./figures/rad.eps}
    \includegraphics[width=\columnwidth]{./figures/ahu_af.eps}
  \vspace{0.25cm}
  \caption{Simulation of the feedback optimization algorithm \protect\eqref{eq:PGM} on the building dynamics~\eqref{eq:1}.}
  \label{fig:feedback_opt_results}
\end{figure}



% paragraph introducing buildings

% The state-of-the-art in building automation is to use model-predictive control (MPC) to control heating and cooling components, such as radiators or air-handling units, to keep the rooms in a building within certain temperature bounds while minimizing energy usage~\cite{drgovna2020all}.
% These methods often rely on white-box or grey-box modeling paradigms, which can be expensive to produce.
% Of recent interest are black-box modeling paradigms in which data is used in lieu of a model, such as \cite{shi2020robust,bunning2020input,hosseinloo2020data}.
% The main drawback with MPC is that computing a solution over long time horizons (i.e., a week) is computationally expensive, and typically limits building automation algorithms to have sampling times of 15-30 minutes in practice.
% Feedback equilibrium seeking allows one to use coarse models to track an equilibrium within a set of constraints, which makes it ideal for a computationally cheaper alternative to regulate room temperatures in buildings~\cite{hauswirthoptimization}.



In this section, we illustrate how FES can be applied to smart building automation. Consider the 5-room single-story office building in Fig.~\ref{fig:building}. Its dynamics\footnote{The model is generated using the BRCM toolbox~\cite{sturzenegger2014brcm}. The bilinearity in \eqref{eq:1} arises from the AHU, whose dynamics include bilinear terms multiplying air flow by the air temperature from the intake (the ambient air temperature), and the outtake (the room temperature).
} can be expressed as,
\begin{equation}\label{eq:1}
    \dot{x} = Ax + B_u u + B_w w + \sum_{i=1}^{n_u} \left(B_{wu,i}w + B_{xu,i}x \right) u_{i}.
\end{equation}
The state $x\in \mc{L}^{113}$ contains the temperatures of the rooms, as well as all other building elements considered by the model, such as wall layers, floor layers, etc. The control inputs $u\in \mc{L}^{8}$ are an air handling unit (AHU) and one radiator in each room. The radiators emit a heat gain between 0 and 50 W/m$^2$, and the AHU inputs are the air flow (0-1kg/s), heating power (0-1000W), and cooling power (0-100W).
We denote the set of these actuation constraints as $\mathcal{U}$.


The disturbances $w\in \mc{L}^{10}$ include the solar radiation, the ambient outdoor air temperature, the temperature of the ground, and the internal heat gains coming from building occupants. The measurement $y\in \mc{L}^{7}$ contains the temperatures of each room as well as the outside air and ground temperatures. Solar radiation and the heat emitted by the buildings occupants are unmeasured, the former since accurately modeling the physics of windows to yield such a measurement is expensive, and the latter due to privacy.

We model 15 building occupants (100W each) by a Markov chain, with a time-dependent probability of being in a given room~\cite{wang2011novel}, and consider an 8 hour work day with a 1.5 hour lunch break. The solar radiation and ambient temperature are modelled via periodic functions yielding temperatures and solar gains representative of central European springtime.

The objective is to minimize energy usage while maintaining the room temperatures within a comfortable range $\mc{T} = [T_{\min}~T_{\max}]$. This is encoded in the following cost
%\begin{subequations}
\begin{align} 
  \varphi_1(u,y) &= \frac{1}{2} (Hu + c)^Tu 
  + \frac{\eta}{2} \sum_{i=1}^{5} {\mathrm{dist}(y_i,\mc{T})}^2 ,\label{eq:2}
%  \\
%  \varphi(u) &= \iota_\mc{U}(u),
%  \label{eq:2_nonsmooth}
\end{align}
%\end{subequations}
where $\eta>0$, $H \succ 0$, and $c$ are weights encoding electricity prices and to ensure strong convexity of the cost, and $\mathrm{dist}(y,\mc{T}) = \min_{u\in \mc{T}} \|y - u\|$ is the distance to the set $\mc{T}$. The actuation limits are modelled by the additional term $\varphi_2(u) = \iota_\mc{U}(u)$, where $\iota_\mc{U}$ is the indicator function of the set $\mc U$. Based on these costs and the steady-state map associated with \eqref{eq:1}, we construct a FO controller using the algorithm described in Sections~\ref{ex:opt_zeros} and \ref{ex:gradient_descent}.
We set $\epsilon=1,\tau=0.05$.

Simulation results are presented in Figure~\ref{fig:feedback_opt_results}.
The controls calculated via FO are able to keep the rooms between the temperature bounds, with only minor constraint violations.
We compare the controller performance to a hysteresis-based thermostat controller, which turns the radiators and AHU heater on when $T_{\text{room}} \leq \frac{T_{\min} + T_{\max}}{2} - 2$ and off when $T_{\text{room}} \geq \frac{T_{\min} + T_{\max}}{2}$. The AHU cooler is turned on when $T_{\text{room}} \geq \frac{T_{\min} + T_{\max}}{2}+2$, and off when $T_{\text{room}} \leq \frac{T_{\min} + T_{\max}}{2}$, with all temperatures in $^\circ$C.
In our example, the FO method provides a 55.15\% reduction in constraint violations, and a 17.99\% reduction in total cost as measured by~\eqref{eq:2}.
A script is available in the \texttt{gitlab} repository\footref{gitlab} demonstrates a set of parameters yielding to instability of the algorithm.




% paragraph outlining results and comparison with hysteresis


%%% Local Variables:
%%% TeX-master: "CDC21.tex"
%%% End:

